Batch Selection and Communication for Active Learning with Edge Labeling

Conventional retransmission (ARQ) protocols are designed with the goal of ensuring the correct reception of all the individual transmitter's packets at the receiver. When the transmitter is a learner communicating with a teacher, this goal is at odds with the actual aim of the learner, which is that of eliciting the most relevant label information from the teacher. Taking an active learning perspective, this paper addresses the following key protocol design questions: (i) Active batch selection: Which batch of inputs should be sent to the teacher to acquire the most useful information and thus reduce the number of required communication rounds? (ii) Batch encoding: Can batches of data points be combined to reduce the communication resources required at each communication round? Specifically, this work introduces Communication-Constrained Bayesian Active Knowledge Distillation (CC-BAKD), a novel protocol that integrates Bayesian active learning with compression via a linear mix-up mechanism. Comparisons with existing active learning protocols demonstrate the advantages of the proposed approach.

==> old/CommTheoryIntro.tex <==
In a classic communication-theoretic model, the sender organizes the data into a set of packets that are then passed on to a lower layer in the protocol stack. The responsibility of the lower layer is to ensure reliable transmission, such that \emph{all} data packets from the sender's set are reliably replicated at the destination. In doing so, the sender runs an Automatic Repeat Request (ARQ) protocol and the destination sends ACK/NACK to indicate the status of the received packets. The packets are sent without replacement, that is, upon reception of ACK, the packet is never sent again. 

Now assume that the sender is a learner that uses a  channel to communicate to a teacher. The packets at the learner are based on data samples that are unlabelled and the learner can send them over the channel to the teacher, which is assumed to be able to label the data. This could be done by using the classic communication-theoretic model from above, such that all $N$ data samples are replicated at the teacher side, say after using an ARQ protocol, and the teacher sends the labels over a feedback channel. We generalize this model by noticing that the communication objective is not replication of the data at the teacher, but a satisfactory learning performance at the learner. This brings two aspects in the model. \emph{First, } if the learner uses active learning, then it does not need to send all $N$ data points, but rather a subset that is sufficient in terms of learning targets. \emph{Second, } the learner does not need to send individual data samples, but rather a mixup of samples. This saves bandwidth over the communication channel, while the teacher could still be able to reliably label the mixup data and thus support the learning objective, without getting clean replicas of the original data from the sender. 



==> old/old.tex <==
% \clearpage\newpage 

% \section*{\colr{Garbage and Pointers}}

% \vc{
% %where the right-most term computes the variance over models in getting the hard estimate $\hat{y}_b$ with $\mathbb{V}$ being the variance operator, whose variance is computed over model parameters. % and  where the higher, the better. 
% The expert's accuracy can be evaluated over a test dataset, $\mathcal{D}_{\rm test}$, as:
% \begin{equation}
%     \mathrm{ACC}^{\rm ex}= \mathbb{E}\left[ \dfrac{\sum_{(\mathbf{x}_i,y_i)\in\{(\mathbf{x}^{\star}_1,y^{\star}_1),\dots,(\mathbf{x}^{\star}_B,y^{\star}_B)\}} \mathbbm{1}_{({y}_i  == \hat{y}_i)}}{B} \right],
%     %\dfrac{\sum_{(\mathbf{x}_i,y_i)\in\mathcal{D}_{\rm test}} \mathbbm{I}({y}_i  == \hat{y}_i)}{|\mathcal{D}_{\rm test}|}
%     \label{eq:expert-accuracy}
% \end{equation}
% where $\mathbbm{1}$ is the indicator variable, and the batches are formed by using a random acquisition function $a$ over $\mathcal{D}_{\rm test}$ without replacement. The expectation is taken concerning the random generation of batches. Note that, in \eqref{eq:hard-estimate} and \eqref{eq:confidence}, the expert's labeling is affected by the distortion, where $\hat{y}_b(\delta_b)$ and $\epsilon_b(\delta_b)$ can be seen as a function of $\delta_b$. Consequently, the expert accuracy also depends on the distortion level, $\mathrm{ACC}^{\rm ex}(\delta_b)$.} We remark the following on this trade-off. %The following interesting trade-off is revealed by noticing this relationship.

% \begin{remark} (Performance-Efficiency Trade-Off) 
%     As the overall compression ratio $R$ decreases, communication cost savings rise, but so does distortion $\delta_b$, leading to reduced accuracy in expert labeling. Consequently, the likelihood of the expert misleading the learner's model and negatively impacting its performance increases. Therefore, considering available channel resources, we must balance compression and learner's performance by carefully designing $\mathbf{P}$, $\mathbf{C}$ and selecting a good compression ratio $R=R_BR_C$.\footnote{We acknowledge that the acquisition function, $a$, has the potential to be optimized for tuning the learner's performance-compression balance of the learner. However, this falls beyond the scope of our current work.}
%     \label{def:misleading-labeling-vs-cost}
% \end{remark}

% % This raises the question of how the expert should handle the received message and labels the data points within the batch. Based on Assumption \ref{assumption:batch-selection}, we assume that the learner intents to receive labeling information for each data point present in the batch. Consequently, the expert's model can be designed in one of two primary ways: 1) Multi-Label Model: In this approach, the expert employs a multi-label model that takes the $\mathbf{t}$ codes as input and produces a vector of labels as output; 2) Classification Model with Decoder: Alternatively, the expert uses a classification model that accepts data points $\mathbf{x}$ and generates a label for a given input. In this case, the expert must incorporate a decoder block to reverse the compression carried out by the learner. The choice between these two designs comes up against the following requirement for the expert feedback message.

% %\noindent\textit{Labeling Ordering Requirement.} From an engineering standpoint, the expert feedback message should have a structured order for associating label information with each data point that comprises the batch. For example, the order in which the batch was stacked together on $\mathbf{X}$ should be the same order in which the label information will return.

% %Because of the above requirement, the multi-label model encounters a problem since developing a way to keep the ordering in the model's output is more complex. Therefore, we will assume that the expert adopts a classification model with a decoder. Because of this, the expert should know the matrices $\mathbf{C}$ and $\mathbf{P}$. In particular, to realize the labeling ordering requirement, we assume that the code matrix $\mathbf{C}$ can be designed to provide an order when combining the data points over the batch dimension. Subsection \ref{sec:practical:code-matrix} will discuss more about this. 


% %which depends on the choice of $\mathbf{C}$ and $\mathbf{P}$. 

% \noindent\colr{
% \textbf{Victor.} Just wondering if it would be nice to present results where those errors are separated or if it is nice to introduce these two types of errors (idea for the future perhaps):
% \begin{remark}
%    % From Assumption~\ref{assumption:informant-expert}, 
%    We distinguish the expert's labeling errors into two categories. Class-I Labeling Error, which occurs independently of communication. Class-II Labeling Error, associated with the learner's Compression method. Our engineering emphasis is on addressing Class-II errors, as Class-I errors are influenced by data and model quality, ratios that are considered beyond our design control.%\footnote{In principle, the expert's model could be trained to be robust against the reconstruction error. But we focus our study on understanding the impact of the reconstruction error in the }
% \end{remark}
% }

% % When designing the 
% % The problem with the first design choice is that multi-label methods lack keeping the relationship between the output labels and the data points in the batch. While the second, this order could obtained by properly design of the matrices $\mathbf{C}$ and $\mathbf{P}$. This order 

% %%%%%
% \subsection{Decision Block}\label{sec:protocol:decision}
% %%%%%
% In traditional \gls{al}, \emph{stopping criteria} commonly involves reaching a predefined target accuracy of the learner's model over a test dataset, $\mathrm{ACC}_{\rm tgt}$ or exhausting the pool dataset, $|\mathcal{U}|=0$. We discard the option of an stopping criteria based on $\mathrm{ACC}_{\rm tgt}$ since we assume the learner lacks a test dataset due to limited memory, necessitating external performance evaluation. Therefore, the decision block incurs the realization of a decision process over \gls{al} loops described in Algorithm \ref{algo:decision-block}, which defines a stopping criteria conspiring the finite number of available channel uses, $C$. %For this reason, we modify the stopping criterion ($|\mathcal{U}|=0$) to consider communication costs.  outlines the learner's decision-making process . 
% Thus, the decision process primarily involves assessing the interaction opportunities between the learner and the expert. The learner stops performing \gls{al} in two ways: i) if the pool dataset is exhausted, the learner does not have any more unlabeled samples to get labels for, and it stops asking; ii) if the communications resources do not allow the realization of another \gls{al} loop, the learner also stops, where the \textit{total communication cost} of an \gls{al} loop is $B^{\prime}D^{\prime}$ according to Subsection~\ref{sec:protocol:transmission}.
% %availability of communication resources for another \gls{al} loop and verifying if the pool dataset has not been exhausted (Algo. \ref{algo:decision-block} -- Step 4). 

% When performing the (iii) retraining step of \gls{al}, to avoid misleading examples, that is, examples with wrong labels, the learner only adds to the training dataset data points whose expert's labeling confidence exceeds a threshold $\epsilon_{\rm th}\in[0,1]$ (Algo. \ref{algo:decision-block} -- Steps 6-12). A \textbf{naive learner} is when we have the zero threshold case, $\epsilon_{\rm th}=0$, where the learner accepts all expert labels. When no more \gls{al} loop can be performed, we consider that an external evaluator estimates the learner's accuracy over a test dataset. 
% % :
% % \begin{equation}
% %     \mathrm{ACC}=\dfrac{1}{|\mathcal{D}_{\rm test}|}\sum_{(\mathbf{x}_i, y_i)\in\mathcal{D}_{\rm test}} \mathbbm{1}_{(y_i == \mathcal{M}(\mathbf{x}_i))},
% %     \label{eq:learner-accuracy}
% % \end{equation}
% % where $\mathcal{M}(\mathbf{x}_i)$ represents that the learner's model has been applied over the data point $\mathbf{x}_i$ and its most average hard-label estimate retrieved as output. 
% The outputs of interest are the final learner's accuracy, $\textrm{ACC}$, the number of \gls{al} loops performed, $L$, and the number of spend channel uses, $C$.



% % \colr{Still working here.}
% % This part discusses how the learner decides whether to proceed with the \gls{al} procedure after receiving the expert feedback message. For a very first study on how the decision process is made, we are going to assume that the batch size %$B,B^{\}$

% % \vc{The decision strategy is comprised of steps.} 

% % Firstly, before updating its training dataset, the learner evaluates the confidence level of the expert labeling of each data point in the batch. Let $\epsilon_{\rm tgt}$ be a target confidence level that measures the learner's willingness to believe in the expert. The learner then performs a confidence check by updating its training dataset solely with the data points that meet the target confidence. Secondly, the learner retrains its model over the updated dataset and estimates its accuracy over a separate local test dataset. With the estimated accuracy, the learned can check if the target accuracy was met. If yes, the learner stops the \gls{al} process; otherwise, the learner proceeds to the next decision step. Thirdly, the learning computes metrics that enable it to evaluate the current \gls{al} loop. The average expert's confidence level is computed as:
% % \begin{equation}
% %     \overline{\epsilon}=\dfrac{1}{B}\sum_{b=1}^{B} \epsilon_b,
% % \end{equation}
% % and it helps the learner to evaluate the impact of compression in Class-II labeling errors on the expert's labeling.

% % \vc{
% % Idea. I am still working here. Not very clear how to design. At first, we could fix $B$ and $B^\prime$ and create a heuristic that keeps tracking $\overline{\epsilon}$ and changes $D$ and $D^\prime$, for example. The idea is that the confidence level is related to the reconstruction error.
% % }



% % After the labeling error correction, the learner retrains its model over the new dataset $\mathcal{L}$, and it is ready to move to a new \gls{al} loop. The learner can stop if a certain performance has been reached or the pool has been extinguished,  $\mathcal{U}=0$. 

% % \TODO{
% % Another idea would be to put a reinforcement learning loop on top of it instead of dealing with the many introduced parameters and the heuristics based on how the parameters' values relate to performance. We could then define a state by using a history of important metrics that can help us to define the trade-off between learner's accuracy and number of channels. 
% % }

% % %%%%%
% % \subsection{Acquisition Step}
% % %%%%%
% % First, the learner as described in \eqref{eq:system-model:acquisition-step} by selecting an acquisition function $a$, \emph{e.g.}, BALD~\cite{Houlsb2011} or BatchBALD~\cite{Kirsch2019}. Inspired by \gls{cdma}~\cite{Verdu1998}, the learner combines the data points by encoding each data point $\mathbf{x}^{\star}_{b}$, which encompasses spreading the data points over its corresponding signature sequence $\mathbf{s}_{c(b)}\in\mathbb{R}^{S}$, where $S$ is the \emph{spreading ratio}. The function $c(b)$ assigns the data point $b$-th to a corresponding signature sequence. Let $\mathbf{S}\in\mathbb{R}^{{S}\times{B}}$ be the matrix containing the signature sequence assigned for each data point in the batch. Thus, the learner gets a \textit{compound data point} $\mathbf{x}\in\mathbb{R}^{L}$ with $L=SN$, whose $n$-th feature dimension is:
% % \begin{equation}
% %     \mathbf{x}_n= \mathbf{S} \underline{\mathbf{x}}_n^{\star},
% %     \label{eq:acquisition-step:cdma-tx}
% % \end{equation}
% % where $\mathbf{x}_n\in\mathbb{R}^{S}_{+}$, $\underline{\mathbf{x}}_n^{\star}\in\mathbb{R}^{B}_{+},\,\underline{\mathbf{x}}_n^{\star}=[{{x}}^{\star}_{1n},{{x}}^{\star}_{2n},\dots,{{x}}^{\star}_{Bn}]^{\transp}$. The compound data point is $\mathbf{x}=[\mathbf{x}_1,\mathbf{x}_2,\dots,\mathbf{x}_N]$.
% % %We define the \emph{spreading ratio} as $R=\frac{L}{N},\, 0\leqR\leq1$. We let $\boldsymbol{\Psi}$ denote the pool of signature sequences, such that $\mathbf{s}_{c(b)}\in\boldsymbol{\Psi}$ and $\ltwonorm{\mathbf{s}_{c(b)}}^2=1$. 

% % \begin{remark}(Non-Orthogonal Signature Sequences).
% %     In principle, the signature sequences $\mathbf{S}$ can comprise orthogonal or non-orthogonal codes. However, using  orthogonal codes would imply that $L=BN$, whose case is equivalent to transmitting each batch data point separately. This goes against our problem statement. Therefore, we are interested in studying non-orthogonal signature sequences, which makes us capable to transmit $B$ data points by using $S<B$ signature sequences.
% %     \label{remark:non-orthogonal}
% % \end{remark}
    
% % %The choice of such and its implication will be discussed in the next section.

% % %%%%%
% % \subsection{Labeling Step}
% % %%%%%
% % We assume that the expert knows the signature sequences, $\mathbf{S}$. The learner transmits the compound data point in eq. \eqref{eq:acquisition-step:cdma-tx} over the \gls{dch}. The expert receives the signal $\mathbf{y}_n\in\mathbf{R}^{S}$ for the $n$-th feature dimension:
% % \begin{equation}
% %     \mathbf{y}_n=\sqrt{\gamma}\mathbf{S} \mathbf{x}_n + \mathbf{n}_n =  \sqrt{\gamma}\mathbf{S} \underline{\mathbf{x}}_n^{\star} + \mathbf{n}_n,
% %     \label{eq:acquisition-step:cdma-rx}
% % \end{equation}
% % where $\gamma\in\mathbb{R}_{+}$ is the \gls{snr} and $\mathbf{n}_n\sim\mathcal{N}(\mathbf{0},\mathbf{I}_{S})$ is \gls{awgn}, which is considered to be \gls{iid} over the feature dimension $n$. The aggregated received signal $\mathbf{y}\in\mathbf{R}^{L}$ is $\mathbf{y}=[\mathbf{y}_1,\mathbf{y}_2,\dots,\mathbf{y}_N]$. Next, the expert sequentially performs the \textit{despreading step} $\hat{x}^{\star}_b=[\mathbf{s}_{c(b)},\mathbf{s}_{c(b)},\dots,\mathbf{s}_{c(b)}]^{\transp}\mathbf{y}$ for the $b$-th data point, where the signature is repeated for $N$ times. When considering the $n$-th dimension, we have
% % \begin{equation}
% %     \hat{x}^{\star}_{bn}=\dfrac{1}{\sqrt{\gamma}}\mathbf{s}_{c(b)}^{\transp}\mathbf{y}_n = {{x}^{\star}_{bn}} + \underbrace{\sum_{i=1,i \neq b}^{B}\mathbf{s}_{c(b)}^{\transp}\mathbf{s}_{c(i)} {x}^{\star}_{in}}_{\text{distortion}} + \underbrace{\vphantom{\sum_{i=1,i \neq b}^{B}}\dfrac{\mathbf{s}_{c(b)}^{\transp}\mathbf{n}_n}{\sqrt{\gamma}}}_{\text{noise}}.
% %     \label{eq:acquisition-step:estimated-signal}
% % \end{equation}
% % In the right-hand side of the above equation, we can see that the original data point ${{x}^{\star}_{n}}$ suffers from two undesirable phenomena. First, the data point is distorted by the other signals in the batch, whose distortion level is proportional to the \gls{crc} level among signature sequences, which is proportional to $\mathbf{s}_{c(b)}^{\transp}\mathbf{s}_{c(i)}$. Second, the signal is degraded by the \gls{awgn}. 

% % After getting all the estimated data points in the batch $\{\hat{\mathbf{x}}^{\star}_{1},\dots,\hat{\mathbf{x}}^{\star}_{B}\}$, the expert uses its model to get a posterior soft labeling estimate for each data point as follows:
% % \begin{equation}
% %     p(\hat{y}_b|\boldsymbol{\theta}^{\prime})=.
% %     \label{eq:acquisition-step:soft-estimate}
% % \end{equation}
% % A hard labeling estimate is given by
% % \begin{equation}

% %     \label{eq:acquisition-step:hard-estimate}
% % \end{equation}
% % where the expectation is taken with respect to the model perimeters $\boldsymbol{\theta}^{\prime}$. 

% % \begin{remark}
% %     The main problem of considering the communication channel in the traditional Bayesian active learning setup is revealed in eq.~\eqref{eq:acquisition-step:soft-estimate}, where one can observe that the data point evaluated by the expert's model now suffers from distortion and noise. Therefore, the expert's model is more likely miss-label the data point.
% %     \label{remark:main-problem}
% % \end{remark}

% % %%%%%
% % \subsection{Retraining Step}
% % %%%%%
% % Retraining starts with the expert responding to the learner over the \gls{fbch}. We consider that the response comprises the hard labeling estimates, as in \eqref{eq:acquisition-step:hard-estimate}, followed by their confidence levels, as in \eqref{eq:acquisition-step:confidence}. The order in which the response is sent is given by the ascending order of the signature sequence indexes so that there is no ambiguity in assigning the responses to the data points in the batch. The idea of sending the confidence levels along with the hard labeling estimates is to use them as an error detection mechanism on the learner side. Thus, before the learner moves to the next \gls{al} loop, the learner can evaluate if it got good enough labeling information from the expert for each data point in the batch. We consider that the learner can deal with the detected errors in two different ways, as described below.

% % \subsubsection{Ignoring Errors (IE)}

% % \subsubsection{Correcting Errors (CE)}
% % Motivated by traditional error correction mechanisms, such as \gls{arq}, we propose that the learner applies a labeling-error correction approach, as described in Algorithm. The idea is that the learner adds to its training data set labels that are correct enough by stipulating a confidence threshold $\epsilon_{\rm th}$, which measures how much the learner is willing to believe in the responses given by the expert. The responses that pass the confidence check are added to the training dataset, while the others are asked again to be labeled by the expert. The loop terminates if a maximum number of iterations is reached or when there is no data point in the batch whose response did not pass the confidence check.



% % %
% % \noindent\textbf{Impact on Average Correct Labeling Throughput} The downside..
% % %



% {\colr{NEED TO BE REVIEWED ACCORDING TO CHANGES IN SECTION 2 and 3. September, 13.}}

% This section will explore specific design choices for the code matrix, $\mathbf{C}$, and the dimensionality reduction matrix, $\mathbf{P}$, introduced in Subsection \ref{sec:protocol:transmission}. At first, the design of these matrices is conducted separately; then, they are analyzed jointly. We evaluate the designs numerically via the performance-efficiency trade-off.
% %To evaluate our designs, this section analyzes the trade-off observed in Remark \ref{def:misleading-labeling-vs-cost}%, which identifies that by having a higher distortion, the expert's performance decays, where the distortion level can be controlled by properly designing $\mathbf{C}$ and $\mathbf{P}$ and selecting the associated hyperparameters $R_B$ and $R_C$. Thus, we conduct numerical simulations to analyze the isolated relationship of certain choices and parameters with performance metrics of interest, which are defined before presenting the designs. 
% The description of our toy example to conduct the simulations is in the Appendix. This section assumes the benchmark case in which the acquisition function, $a$, in eq. \eqref{eq:system-model:acquisition-step} selects random data points from the pool dataset without replacement to comprise the batch. 

% %%%%%
% \subsection{Performance Metrics}
% %%%%%
% \vc{
% To evaluate how the distortion impacts the expert's performance, we would like to measure how much the performance of the expert degrades as a function of the distortion, which is in its turn stipulated by the design of the matrices $\mathbf{C}$ and $\mathbf{P}$ and the hyperparameters $R_B$ and $R_D$. Thus, we establish contrasting loss metrics between the expert's performance with and without compression, where the word. First, let $\mathrm{ACC}^{\rm ex}_{\rm up}$ be the expert's upper bound in performance when there is no distortion. We define the \emph{expert's accuracy loss} as:
% \begin{equation}
%     \text{expert's accuracy loss}=\dfrac{\mathrm{ACC}^{\rm ex}_{\rm up}-\mathrm{ACC}^{\rm ex}}{\mathrm{ACC}^{\rm ex}_{\rm up}},
% \end{equation}
% where the accuracies are computed as in eq. \eqref{eq:expert-accuracy}. This metric quantifies the decrease in expert accuracy resulting from distortion. Second, similarly, let $\epsilon_{b,\rm up}$ be the expert's upper bound in labeling confidence. We define the \emph{expert's labeling confidence loss} as:
% \begin{equation}
%     \text{relative expert's labeling confidence loss}=\dfrac{\epsilon_{b,\rm up}-\epsilon_{b}}{\epsilon_{b,\rm up}}
% \end{equation}
% where the labeling confidence is computed as in eq. \eqref{eq:confidence}. This metric tells us how less confident the expert is in labeling due to distortion. Both metrics range between $[0,1]$.%; the lower, the better.
% }
% % A generic formulation of a relative loss metric is given by:
% % \begin{equation}
% %     \text{relative loss metric} = \dfrac{\text{w/o comp.} - \text{w/ comp.}}{\text{w/o comp.}}.
% %     \label{eq:relative-metric}
% %\end{equation}


% %Based on the above, we define the  and \emph{relative expert's confidence loss}. The relative loss metrics provide insights into the extent to which the expert's labeling ability is compromised by compression, where the higher the relative loss metrics, the poorer the experts' performance; consequently, the expert would mislead the learner to a greater extent.

% %tell us how much of the performance of the expert is preserved after compression is applied. Thus, the relative metrics are a function of the $R_B$ and $R_D$ compression ratios.
% % \begin{remark}
% %     A benchmark for relative accuracy is the unity line, in which the relative accuracy decreases at a one-to-one rate with the compression ratio. This means we compress as much as we lose in the expert's performance. We want to reach curves in which the loss in the expert's performance decreases slowly with the compression ratio; we are looking for a Compression method whose curve is in the region over the unity line.
% %     \label{remark:benchmark}
% % \end{remark}

% %%%%%
% \subsection{Code Matrix Design}\label{sec:practical:code-matrix}
% %%%%%
% The design of the code matrix should remain data-independent since one batch is selected at a given \gls{al} loop, as in \eqref{eq:system-model:acquisition-step}, and batch selection is dependent on the learner's model, which changes over \gls{al} loops, preventing us from statistically analyzing data over the batch dimension for compression purposes. \vc{Hence, we adopt the design principle of employing transform coding~\cite{Salomon2008} as our approach. Specifically, our idea revolves around selecting a set of sequences denoted as $\{\underline{\mathbf{c}}^{\transp}_b\}_{b=1}^{B}$, where each sequence $\underline{\mathbf{c}}^{\transp}_b$ resides in $\mathbb{R}^{B^\prime}$ and possesses a unit norm, $\lVert\underline{\mathbf{c}}^{\transp}_b\rVert^2_2=1$. These sequences are strategically chosen to span the $B^{\prime}$-dimensional space onto which the batch will be transformed. Their primary role is linearly combining the $B$ data points, effectively projecting them into the lower-dimensional space.
% }

% \vc{
% These selected sequences must facilitate high-quality reconstruction when transforming the batch to its original form, akin to image "upscaling." Notably, since the downscaled dimension $B^{\prime}$ is less than the original dimension $B$, the selected sequences cannot be orthogonal to each other. Instead, it is crucial that these sequences exhibit robust Cross-Representation Coherence (CRC) properties. The CRC between any two sequences can be mathematically defined as follows:
% \begin{equation}
%     \mathrm{CRC}_{b,b^{\prime}}=(\underline{\mathbf{c}}^{\transp}_b)^{\transp}(\underline{\mathbf{c}}^{\transp}_{b^{\prime}}).
% \end{equation}
% Drawing from the extensive literature on compression techniques~\cite{Salomon2008}, we have a diverse pool of sequence sets to choose from. These sets include sequences based on cosine functions, polynomials, spherical harmonics, Bessel functions, and wavelets. The selection of the most suitable sequence set depends on the specific properties and characteristics of the batch data, allowing us to tailor our choice to the application's requirements. Once again, due to the challenges of statistically analyzing the batch dimension, we opt for generic choices and rely on practical evaluation.}

% %Our proposed design for the code matrix is inspired by the idea of non-orthogonal \gls{cdma} for multiple users, where different sequences with tunable \gls{crc} are assigned to users, enabling multi-user communication~\cite{Bertsekas1996}. Our idea then was to interpret data points within a batch as users and find a $\mathbf{C}$ with . However, different from \gls{cdma}, where the data from the users are spread over sequences, the data from the data points in the batch are shrunk over sequences. Hence, we must, in principle, not utilize the same types of sequences used for \gls{cdma}, such as Walsh or Gold codes. Then, we have designed $\mathbf{C}$ based on codes used in the compression literature~\cite{}.

% % In Section~\ref{sec:protocol}, the main design principles observed for $\mathbf{C}$ are that i) it should ensure the label ordering requirement and ii) the design of $\mathbf{C}$ should be independent of data since the \gls{al} loop does not enable us to statically analyze the batch dimension as we chose a batch per \gls{al} loop to be sent. Given these two requirements, we have been inspired by the idea of non-orthogonal \gls{cdma} for multiple users to design $\mathbf{C}$ as a code matrix comprised of multiple sequences with tunable \gls{crc}. An assignment function then assigns each sequence to each data point in the batch, ensuring the label ordering requirement since the expert also knows the $\mathbf{C}$ before communication. For example, in a round-robin fashion, the first data point would be assigned to the first sequence, and so on. Therefore, we can control how much each data point in the batch interferes with each other by carefully designing the sequences, where the sequence \gls{crc} would be ultimately linked to the reconstruction error, $R_b$. 

% To showcase the design of the code matrix $\mathbf{C}$, we choose the following two codes: 1) Gaussian Codes: As a baseline scheme, we consider Gaussian-generated codes where we have little control over the \gls{crc}; 2) \Gls{rdft}: A widely-used compression matrix in various applications with real data~\cite{Salomon2008}, the real \gls{rdft} has good \gls{crc} properties. 
% %By letting each sequence $\underline{\mathbf{c}}^{\transp}_b\in\mathbb{R}^{B^\prime}$ in $\mathbf{C}$ have unit norm $\lVert\underline{\mathbf{c}}^{\transp}_b\rVert^2_2=1$, we evaluate a design $\mathbf{C}$ by characterizing the properties of the \gls{crc} between two sequences, given by:
% % \begin{equation}
% %    \mathrm{CRC}_{b,b^{\prime}}=(\underline{\mathbf{c}}^{\transp}_b)^{\transp}(\underline{\mathbf{c}}^{\transp}_{b^{\prime}}).
% % \end{equation}
% % The higher the average \gls{crc}, the higher the distortion among data points in a batch; consequently, the worse the expert's performance will be.

% %The $\mathrm{CRC}_{b,b^{\prime}}$ is a random variable, and we are interested in characterizing its properties.

% In Figure~\ref{fig:code-matrix}, we assess two distinct code matrix designs, yielding the following observations. 1) The Gaussian code matrix exhibits a notably high \gls{crc}, leading to significantly elevated distortion levels in comparison to the \gls{rdft}. 2) The \gls{rdft} demonstrates that effective compression can be achieved with minimal loss in accuracy. For instance, with $B=32$, we can save 30\% ($R_B=70\%$) of channel resources while only reducing expert accuracy by 14\%. 3) As batch size $B$ increases, the average \gls{crc} decreases, resulting in improved overall performance. However, there is an increase in result variability, indicating a limit to how much we should increase $B$ since excessive variability can impact the \gls{al} loops that are executed online.

% \vc{\textbf{Victor.} A possible problem with using DCT is that it assumes periodicity (cosine is periodic) among batches; this is not true since we expect batches to have different data points, that is, contents (different images in the MNIST case). We could try some wavelet codes, or Bessel functions to see if we get some improvement if necessary.}

% %nd drastically impacting the performance of the expert, where for some batch compression values, we have performances lower than the unity line (see Remark~\ref{remark:benchmark}). On the contrary, we observe that the \gls{rdft} code matrix design ensures us relative performance metrics close or as close to the unity line, satisfying the requirement of at least achieving a one-to-one-linear relationship between relative expert's accuracy and batch compression ratio.

% \begin{figure*}[t]
%   \centering
%   \subfloat[Gaussian code matrix.]{\includegraphics[width=0.5\textwidth]{figs/gaussian.pdf}}
%     %\hspace{-0.001mm}
%   \subfloat[\gls{rdft} code matrix.]{\includegraphics[width=0.5\textwidth]{figs/real_dft.pdf}}
%   \caption{
%     Average evaluation of different code matrix designs. The \gls{crc} has been averaged over $R_B$, and \gls{crc} plots show the lower and upper quartiles. For accuracy loss, we have included a "reference line, $h(z)=1-z$" to help comparison. This reference line illustrates, for instance, that when utilizing only $R_B=10\%$ of the batch resources, we should anticipate a corresponding 90\% reduction in the expert's accuracy. Our objective is to focus on results within the region below the reference line, where we achieve greater savings while incurring minimal degradation in expert performance.
%     }
%   \label{fig:code-matrix}
% \end{figure*}

% % \begin{table*}[]
% %     \caption{Code Matrix Mean \gls{crc} Between Quartiles}
% %     \centering
% %     \label{tab:code-matrix:crc}
% %     %\resizebox{\columnwidth}{!}{%
% %     \begin{tabular}{cccccc}
% %     \hline
% %     \begin{tabular}[c]{@{}c@{}}Code\\ Matrix\end{tabular} & \multicolumn{5}{c}{Batch Size} \\ \cline{2-6} 
% %     & 2    & 4   & 8   & 16   & 32   \\ \hline
% %     Gaussian  & (-0.69,0.04,0.68) & (-1.07,0.03,1.17) & (-0.02,0.04,0.68) &      (-0.69,0.04,0.68) &      \\
% %     RDFT  & ()     &     &     &      &     
% %     \end{tabular}%
% %     %}
% % \end{table*}


% %%%%%
% \subsection{Dimensionality Reduction Design}\label{sec:practical:dim-matrix}
% %%%%%
% \vc{
% Unlike the code matrix, the dimensionality reduction matrix $\mathbf{P}$ can be data-driven, relying on analysis of the training datasets of either the learner or the expert. However, given the limited data often available to the learner, we assume that $\mathbf{P}$ is computed by the expert and shared with the learner before starting the batch \gls{al} process. The design principle of the dimensionality reduction matrix, $\mathbf{P}$, is based on the manifold assumption, which dictates that high-dimensional data can be effectively represented in the lower dimensional space~\cite{Bishop2006}. In particular, we employ \gls{pca}, a well-known technique that maximizes the variance of the data project into the lower dimensional space.} 

% Fig.~\ref{fig:dim-matrix} evaluates the \gls{pca} design as a function of the compression ratio over features. In the toy example, we observe that the expert can still utilize a very small subset of features, as some are noise or irrelevant to the classification problem. Notably, a sharp performance shift occurs at the point $D^{\prime}=32$ and $R_D=0.04$; at this point, \gls{pca} explains approximately 75\% of the data variance. 

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/pca.pdf}
%     \caption{Average evaluation of dimensionality reduction matrix based on \gls{pca}.}
%     \label{fig:dim-matrix}
% \end{figure}

% %We design , by using \gls{pca}~\cite{}. Before \gls{al}, we assume that the expert performs \gls{pca} over its training dataset and shares the encoding matrix $\mathbf{P}$ to the learner since the expert has a larger training dataset than the learner. We chose this approach because the learner has a limited dataset, and performing \gls{pca} at its side would result in poor compression performance. 

% %%%%%
% \subsection{\vc{Joint Analysis of the Batch and Feature Compression}}\label{sec:practical:joint}
% %%%%%
% In this section, we examine the joint performance of the designs. Initially, we consider the dimensionality reduction matrix, $\mathbf{P}$, as a constant by setting $D^{\prime}=32$ and $R_D=0.04$. %This choice aligns with practical considerations, as altering $\mathbf{P}$ frequently is undesirable since the expert computes $\mathbf{P}$, necessitating communication with the learner whenever changes are made. 
% Fig.~\ref{fig:joint-matrix} shows the performance when varying the compression ratio over batches, $R_B$ and batch sizes, $R$. Compared to Figure~\ref{fig:code-matrix}, the expert's accuracy shows an average improvement of 12\% for $B=32$ data points, where the average is taken over $R_B$. This enhancement can be attributed to the dimensionality reduction applied over features, resulting in the code matrix combining more pertinent information for classification. Additionally, it helps to prevent the inclusion of augmented noise data that might occur when encoding across the batch dimension.

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/joint.pdf}
%     \caption{Joint average evaluation of the designed code and dimensionality reduction matrices. The code matrix adopts the \gls{rdft} design.}
%     \label{fig:joint-matrix}
% \end{figure}

% %\vc{The idea of these results is to fix the PCA matrix and evaluate how much we can compress by doing joint compression while varying $B$ and $R_B$.}


% % %%%%%
% % \subsection{Correct Labeling Rate and Throughput}
% % %%%%%
% % To capture the learner's goal and measure the protocol's efficiency, we introduce the concept of the \textit{average correct labeling rate} $\overline{R}\in\mathbb{R}_{+}$, which measures the average amount of correct labels being added to the training dataset per active learning round. Mathematically, the average correct labeling rate $\overline{R}$ is
% % \begin{equation}
% %     \overline{R}=\mathbb{E}\left[\sum_{b=1}^{B} \mathbbm{1}_{\{\hat{y}_b = {y}^{\star}_b\}}\right],\,0\leq~\overline{R}\leq B,
% %     \label{eq:problem-statement:avg-correct-labeling-rate}
% % \end{equation}
% % where $\hat{y}_b\in\{0,1,\dots,K-1\}$ is the hard labeling estimate given by the expert's model and ${y}^{\star}_b$ is the true label for the $b$-th data point. The expectation is taken with respect to channel and noise realizations and over the expert's model parameters. The \textit{average correct labeling throughput}, $\overline{T}\in\mathbb{R}_{+}$, can then be computed as 
% % \begin{equation}
% %     \overline{T}=\dfrac{1}{(L+I)}\overline{R},
% %     \label{eq:problem-statement:avg-correct-labeling-throughput}
% % \end{equation}
% % accounting for the number of channel uses spent to get the labels. 

% % \begin{remark}(Relevant Throughput Bounds). 
% %     We consider two relevant bounds for ideal throughput; that is, when all the labels are obtained correctly with the maximum rate being obtained $\overline{R}=B$. \textbf{1) Ideal AL:} first, a baseline bound $\overline{T}_{\rm IAL}\in\mathbb{R}_{+}$ which represent the ideal \gls{al} setup considered so far in the literature in which the learner explicitly transmits all the data points in the batch, $L=BN$, and the expert's answer with the true hard estimates ${y}^{\star}_b$'s, $I=B$. In this case, the throughput evaluates to $\overline{T}_{\rm IAL}={1}/{N}$. However, this bound is impractical since the communication channels and the expert's model can introduce errors when considering the application of interest. \textbf{2) Target:} second, a target bound $\overline{T}_{\rm target}\in\mathbb{R}_{+}$ which corresponds to the case that the $B$ data points are transmitted using the size of a unique data point $N$ and, even so, the expert can perfectly recognize each of the $B$ data points by reversing the signal processing technique applied by the learner and, subsequently, labels them correctly; thus, $\overline{T}_{\rm target}=B/(N+B)$.  
% %     \label{remark:throughput-bounds}
% % \end{remark}

% % %%%%%
% % \subsection{Impact of Noise and Distortion}
% % %%%%%
% % In this part, we evaluate how the distortion and noise 

% % %%%%%
% % \subsection{Expert's Model Training}
% % %%%%%
% % As discussed in the next section, one way to solve the above remark is to carefully train the expert's model to be robust to distortion and noise, \emph{e.g.}, one can use \textit{data augmentation} techniques while training the expert's model.

% % %============================
% % \section{Designing Learner Decision Strategy}
% % %============================

% % %%%%%
% % \subsection{Baselines}
% % %%%%%
% %We define the following \gls{al} strategies as baselines. \noindent\textbf{Conventional \gls{al} Baseline.} This baseline disregards communication costs and assumes a maximum number of \gls{al} loops provided by $\lceil\frac{|\mathcal{U}|}{B}\rceil$. 

% %   \label{definition:baseline2}
% %\end{definition}
% % %%%%%
% % \subsection{Learner's End Performance}
% % %%%%%

